Disentangling the Complex Multiplexed DIA Spectra in De Novo Peptide Sequencing

Data-Independent Acquisition (DIA) was introduced to improve sensitivity to cover all peptides in a range rather than only sampling high-intensity peaks as in Data-Dependent Acquisition (DDA) mass spectrometry. However, it is not very clear how useful DIA data is for de novo peptide sequencing as the DIA data are marred with coeluted peptides, high noises, and varying data quality. We present a new deep learning method DIANovo, and address each of these difficulties, and improves the previous established systems by a large margin, via equipping the model with a deeper understanding of coeluted DIA spectra. This paper also provides criteria about when DIA data could be used for de novo peptide sequencing and when not to by providing a comparison between DDA and DIA, in both de novo and database search mode. We find that while DIA excels with narrow isolation windows on older-generation instruments, it loses its advantage with wider windows. However, with Orbitrap Astral, DIA consistently outperforms DDA due to narrow window mode enabled. We also provide a theoretical explanation of this phenomenon, emphasizing the critical role of the signal-to-noise profile in the successful application of de novo sequencing.

==> chapters/author_contrubition.tex <==

Zheng Ma, Zeping Mao, Ruixue Zhang, Ming Li, and Ali Ghodsi designed research; Zheng Ma, Zeping Mao, Ruixue Zhang, and Jiazhen Chen performed research experiments; Zheng Ma and Zeping Mao contributed new analytic tools; Zheng Ma, Zeping Mao, and Ruixue Zhang analyzed data; and Zheng Ma, Zeping Mao, Jiazhen Chen and Ming Li wrote the paper.

==> chapters/significance.tex <==
Mass spectrometry enables the identification of proteins, which is essential for understanding health and disease. A major challenge lies in de novo peptide sequencing—determining protein fragments without relying on known databases—especially when using data-independent acquisition (DIA), where signals from many peptides overlap with substantial noise. We introduce DIANovo, a deep learning method specifically designed to disentangle these complex DIA spectra. Our theoretical analysis demonstrates that identification performance depends critically on the absolute strength of signal peaks, not just the signal-to-noise ratio. By providing both a practical algorithm and a theoretical framework, we establish when DIA should be used for de novo sequencing, enabling more reliable proteome analysis, biomarker discovery, and personalized medicine applications.


==> chapters/supporting_content.tex <==
\begin{itemize}

\item{Section A – The DIANovo Model.} A detailed description of the proposed de novo sequencing model for DIA.

\item{Section B – Theoretical Analysis.} Simulation design, XCorr computation and exact p-value computation, multiple-hypothesis adjustment and derived relationships for peptide recall and database identification.

\item{Section C – Additional Spectrum Features.} Definitions of eight auxiliary features (normalized m/z, relative intensity, rank/half-rank, local significance, local rank/half-rank, local relative intensity).

\item{Section D – Ion Offsets.} Offsets used to convert ions to N-terminal masses (Supporting Table 1).

\item{Section E – Labeled Ion Types in Pretraining.} Ion types and charge handling for the pretraining labels (Supporting Table 2).

\item{Section F – Precursor Feature Detection.} Feature detection pipelines; fields recorded per feature.

\item{Section G – Characteristics of Test Datasets.} Summary metrics per dataset in Supporting Table 3.

\item{Section H – Links to Datasets.} Access links for all training/testing datasets in Supporting Table 4.

\item{Section I – Model Implementation Details.} Model and training hyperparameters; train/test separation policy.

\item{Section J – Sensitivity to Coelution Number.} Performance versus coelution count (Supporting Figure 1).

\item{Section K – Ablation Study.} Quantitative impacts of components of the model (Supporting Figure 2).

\item{Section L – Visualization of Learned Embeddings.} t-SNE of peak embeddings colored by ion type and by ion source (coeluting peptide) (Supporting Figures 3–5).
\end{itemize}
